Beyond Shadows: A Large-Scale Benchmark and Multi-Stage Framework for High-Fidelity Facial Shadow Removal

Facial shadows often degrade image quality and the performance of vision algorithms. Existing methods struggle to remove shadows while preserving texture, especially under complex lighting conditions, and they lack real-world paired datasets for training. We present the Augmented Shadow Face in the Wild (ASFW) dataset, the first large-scale real-world dataset for facial shadow removal, containing 1,081 paired shadow and shadow-free images created via a professional Photoshop workflow. ASFW offers photorealistic shadow variations and accurate ground truths, bridging the gap between synthetic and real domains. Deep models trained on ASFW demonstrate improved shadow removal in real-world conditions. We also introduce the Face Shadow Eraser (FSE) method to showcase the effectiveness of the dataset. Experiments demonstrate that ASFW enhances the performance of facial shadow removal models, setting new standards for this task.

==> figtex/fig3.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=1\columnwidth]{figs/tsne.pdf}
\caption{T-SNE visualization of input and target images across datasets. ASFW shows closer alignment compared to synthesized data.}
\label{fig3}
\vspace{-10pt}
\end{figure}

==> figtex/fig4.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth]{figs/vis2.pdf}
\caption{Qualitative results on the ASFW dataset. Our method achieves high-fidelity shadow removal compared to state-of-the-art methods.}
\label{fig4}
\vspace{-15pt}
\end{figure*}

==> figtex/fig5.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figs/shadow_distribution.pdf}
\caption{Data diversity distribution of ASFW.}
\label{fig5}
\end{figure*}


==> figtex/fig7.tex <==
\begin{figure}[h]
	\centering
	% \hspace{5mm}
	\begin{minipage}[b]{\textwidth}
	\subfigure[Input]{
		\begin{minipage}[b]{0.16\textwidth}
			\includegraphics[width=0.95\textwidth]{figs/fig2/Input609.png}\\ 
			\includegraphics[width=0.95\textwidth]{figs/fig2/Input612.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/Input629.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/Input638.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/Input713.png}\\
                \includegraphics[width=0.95\textwidth]{figs/fig2/Input760.png}\\
                \includegraphics[width=0.95\textwidth]{figs/fig2/Input9156-004.png}\\
		\end{minipage}
	}\hspace{-3mm}
	%\quad
	\subfigure[HomoFormer]{
		\begin{minipage}[b]{0.16\textwidth}
		    \includegraphics[width=0.95\textwidth]{figs/fig2/HomoFormer609.png}\\ 
			\includegraphics[width=0.95\textwidth]{figs/fig2/HomoFormer612.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/HomoFormer629.png}\\
                \includegraphics[width=0.95\textwidth]{figs/fig2/HomoFormer638.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/HomoFormer713.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/HomoFormer760.png}\\
                \includegraphics[width=0.95\textwidth]{figs/fig2/HomoFormer9156-004.png}\\
		\end{minipage}
	}\hspace{-3mm}
	%\quad
	\subfigure[SG]{
		\begin{minipage}[b]{0.16\textwidth}
		    \includegraphics[width=0.95\textwidth]{figs/fig2/SG_ShadowNet609.png}\\ 
			\includegraphics[width=0.95\textwidth]{figs/fig2/SG_ShadowNet612.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/SG_ShadowNet629.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/SG_ShadowNet638.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/SG_ShadowNet713.png}\\
                \includegraphics[width=0.95\textwidth]{figs/fig2/SG_ShadowNet760.png}\\
                \includegraphics[width=0.95\textwidth]{figs/fig2/SG_ShadowNet9156-004.png}\\
		\end{minipage}
	}\hspace{-3mm}
	%\quad
	\subfigure[ShadowFormer]{
		\begin{minipage}[b]{0.16\textwidth}
		    \includegraphics[width=0.95\textwidth]{figs/fig2/ShadowFormer609.png}\\ 
			\includegraphics[width=0.95\textwidth]{figs/fig2/ShadowFormer612.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/SG_ShadowNet629.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/ShadowFormer638.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/ShadowFormer713.png}\\
                \includegraphics[width=0.95\textwidth]{figs/fig2/ShadowFormer760.png}\\
                \includegraphics[width=0.95\textwidth]{figs/fig2/ShadowFormer9156-004.png}\\
		\end{minipage}
	}\hspace{-3mm}
	%\quad
	\subfigure[Ours]{
		\begin{minipage}[b]{0.16\textwidth}
		    \includegraphics[width=0.95\textwidth]{figs/fig2/Ours609.png}\\ 
			\includegraphics[width=0.95\textwidth]{figs/fig2/Ours612.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/Ours629.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/Ours638.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/Ours713.png}\\
                \includegraphics[width=0.95\textwidth]{figs/fig2/Ours760.png}\\
                \includegraphics[width=0.95\textwidth]{figs/fig2/Ours9156-004.png}\\
		\end{minipage}
	}\hspace{-3mm}
	%\quad
	\subfigure[GT]{
		\begin{minipage}[b]{0.16\textwidth}
   	 	  \includegraphics[width=0.95\textwidth]{figs/fig2/Target609.png}\\ 
			\includegraphics[width=0.95\textwidth]{figs/fig2/Target612.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/Target629.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/Target638.png}\\
			\includegraphics[width=0.95\textwidth]{figs/fig2/Target713.png}\\
                \includegraphics[width=0.95\textwidth]{figs/fig2/Target760.png}\\
                \includegraphics[width=0.95\textwidth]{figs/fig2/Target9156-004.png}\\
		\end{minipage}
		}
	\end{minipage} 
    \vspace{-3mm}
	\caption{Visual comparison of facial shadow removal on ASFW and UCB dataset.} 
	\vspace{-3mm}
	\label{fig:result_comparison2}
\end{figure}

==> figtex/supp1.tex <==
\begin{figure*}
\centering
\includegraphics[height=.95\textheight]{figs/figsupp/supp_1.pdf}
\caption{More Visualization}
\label{supp:fig1}
\end{figure*}


==> figtex/supp2.tex <==
\begin{figure*}
\centering
\includegraphics[height=.95\textheight]{figs/figsupp/supp_2.pdf}
\caption{More Visualization}
\label{supp:fig2}
\end{figure*}


==> figtex/supp3.tex <==
\begin{figure*}
\centering
\includegraphics[height=.95\textheight]{figs/figsupp/supp_3.pdf}
\caption{More Visualization}
\label{supp:fig3}
\end{figure*}


==> figtex/supp4.tex <==
\begin{figure*}
\centering
\includegraphics[height=.95\textheight]{figs/figsupp/supp_4.pdf}
\caption{More Visualization}
\label{supp:fig4}
\end{figure*}


==> sec/2_related.tex <==
\section{Related Work}

\subsection{Facial Shadow Removal}

Early shadow removal methods primarily relied on hand-crafted cues such as chromaticity, gradient consistency, and textural contrast to distinguish shadowed regions~\cite{yang2012shadow, gryka2015learning}. While effective under simple lighting, these techniques struggle with complex occlusions and non-uniform illumination.

With the rise of deep learning, data-driven approaches have significantly advanced shadow removal. Models such as StackedCNN~\cite{wang2018stacked}, and DC-ShadowNet~\cite{jin2021dc} introduced mask-guided and adversarial learning strategies to address shadow detection and removal, often trained on generic scenes. More recent methods like Homoformer~\cite{xiao2024homoformer} and ShadowRefiner~\cite{dong2024shadowrefiner} enhance feature regularization and frequency-domain modeling, respectively, marking a shift toward more robust and generalizable solutions.

However, facial shadow removal remains uniquely challenging due to the complex interaction between facial geometry and lighting. Shadows often occlude semantically important regions such as the eyes, nose, and mouth, leading to degradation in both perceptual quality and downstream recognition tasks~\cite{zhang2020portrait}. Addressing these challenges requires domain-specific designs. Portrait ShadowNet~\cite{zhang2020portrait} introduced dual branches to handle external occlusions and lighting imbalances, while Liu~\etal~\cite{liu2022blind} proposed a grayscale-to-color pipeline to address subsurface scattering artifacts. Recent architectures such as GraphFFNet~\cite{zhang2023facial}, FSRNet~\cite{zhang2024frequency}, and CIRNet~\cite{yu2024portrait} incorporate facial topology, frequency decomposition, and background-aware refinement to preserve identity and structural consistency.

Despite these advances, most methods rely heavily on synthetic datasets, limiting their real-world performance. This highlights the need for high-fidelity, paired facial datasets and facial-aware refinement strategies—core motivations behind our proposed method.


\subsection{Facial Shadow Removal dataset}
Collecting a large-scale dataset of paired images containing face shadows and no shadows requires tedious manual work. The UCB dataset~\cite{zhang2020portrait} is a real-world facial shadow dataset, containing 100 pairs of face images with and without shadows. Since it is real data, it has high credibility and reliability in real-world scenarios. However, the scale of this dataset is relatively small, with only 100 pairs of images. When training complex deep learning models, it may not provide enough data to fully train the model, resulting in limited generalization ability of the model. The generation method of the synthesized datasets is relatively simple, and a large amount of shadow image data can be quickly obtained, which can meet the data volume requirements to a certain extent. However, there are obvious differences in the data distribution of the real world, and the synthesized shadow effect may not be realistic enough, resulting in poor performance of the model trained based on this dataset in actual application scenarios. Photoshop shadow rendering plug-in is currently widely used in professional photo editing and visual effects production, and is very suitable for generating realistic and diverse facial shadows. With the help of advanced shadow rendering plugins in Adobe Photoshop~\cite{adobephotoshop}, we simulate diverse and photorealistic shadow conditions. Our dataset is specifically designed to bridge the domain gap and increase diversity, providing a high-quality resource for training and evaluating robust facial shadow removal models.

==> sec/7_limitation.tex <==
\section{Limitation}
While ASFW offers high-resolution, perceptually aligned shadow/shadow-free facial pairs and addresses common limitations of synthetic data, it remains fundamentally a 2D image-based dataset, which lacks physically accurate light transport modeling based on 3D facial geometry. Nevertheless, this design enables scalable and pixel-aligned data generation for in-the-wild settings, where obtaining ground-truth 3D information is often unavailable or difficult. Future work could explore hybrid strategies that combine the realism of physically-based rendering with the scalability and annotation precision of our 2D framework.

==> tabletex/table1.tex <==
\begin{table}[ht]
\centering
\small
{
\begin{tabular}{l|cc|cc}
\toprule
\textbf{Metric} & \multicolumn{2}{c|}{\textbf{Shadowed}} & \multicolumn{2}{c}{\textbf{Shadowed-free}}  \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} 
 & \textbf{Synth.} & \textbf{Ours} & \textbf{Synth.} & \textbf{Ours} \\
\midrule
Cosine Similarity & 0.6965 & \textbf{0.7449} & 0.7726 & \textbf{0.7982} \\
KID (Std) & 0.0067 & \textbf{0.0026} & 0.0043 & \textbf{0.0029} \\
FID & \textbf{1.3226} & 2.6983 & 2.9935 & \textbf{2.8911} \\
KID (Mean) & 0.1975 & \textbf{0.0607} & 0.0795 & \textbf{0.0754} \\
\bottomrule
\end{tabular}
}
\caption{Comparison of image fidelity metrics between Synthesized and Ours under both Shadowed and Shadowed-free conditions. Metrics are grouped and split for better horizontal comparison.}
\label{table1}
\end{table}

==> tabletex/table4.tex <==
\begin{table}[ht]
    \centering
    \small % 适当缩小字体
    \setlength{\tabcolsep}{5pt} % 调整列间距
    \renewcommand{\arraystretch}{1.3} % 增加行间距
    \begin{tabular}{lccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{ASFW}} \\
        \cmidrule(lr){2-4} 
         & DBCNN $\uparrow$ & NIQE $\downarrow$ & MUSIQ $\uparrow$ \\
        \midrule
        PSM~\cite{zhang2020portrait}  & 0.45 & 5.66 & 60.37 \\
        BlindShadow~\cite{liu2022blind} & 0.48 & 4.98 & 64.06 \\
        Lyu \etal~\cite{lyu2022portrait} & 0.49 & 4.87 & 63.73 \\
        FSRNet~\cite{zhang2024frequency} & 0.50 & 5.01 & 64.56 \\
        CIRNet~\cite{yu2024portrait} & 0.50 & 5.01 & 64.69 \\
        \midrule
        \textbf{Ours} & \textbf{0.51} & \textbf{4.85} & \textbf{64.79} \\
        \bottomrule
    \end{tabular}
    \caption{Supplemental quantitative comparison on ASFW dataset.}
    \label{table4}
\end{table}


==> tabletex/table5.tex <==
\begin{table}[ht]
    \centering
    \renewcommand{\arraystretch}{1.2} % 调整行距
    \setlength{\tabcolsep}{4pt} % 调整列间距
    \resizebox{\linewidth}{!}{ % 适应单栏排版
    \begin{tabular}{l c c c c}
        \toprule
        \textbf{Method} & \textbf{Shadow Region} & \textbf{Shadow Removal} & \textbf{Texture} & \textbf{Non-Shadow} \\
        & \textbf{Localization Accuracy} & \textbf{Naturalness} & \textbf{Consistency} & \textbf{Preservation} \\
        \midrule
        \textbf{HomoFormer}~\cite{xiao2024homoformer}  & 2.82 & 2.66 & 2.72 & 2.72\\ 
        \textbf{PSM}~\cite{zhang2020portrait} & 2.99 & 2.85 & 2.89 & 2.90\\ 
        \textbf{S3RNet}~\cite{kubiak2024s3r}     & 3.16 & 3.00 & 3.09 & 3.12\\ 
        \textbf{SG-ShadowNet}~\cite{wan2022style}    & 2.66 & 2.50 & 2.47 & 2.49\\
        \textbf{BlindShadow}~\cite{liu2022blind}    & 3.29 & 3.08 & 3.16 & 3.17 \\ 
        \textbf{CIRNet}~\cite{yu2024portrait}    & 3.31 & 3.15 & 3.25 & 3.25 \\ 
        \textbf{FSRNet}~\cite{zhang2024frequency}    & 3.37 & 3.20 & 3.26 & 3.24\\ 
        \textbf{Lyu \etal}~\cite{lyu2022portrait} & 3.41 & 3.28 & 3.28 & 3.32\\ 
        \textbf{Ours}    
        & \textbf{\textcolor{red}{4.20}}  
        & \textbf{\textcolor{red}{4.23}}  
        & \textbf{\textcolor{red}{4.16}}  
        & \textbf{\textcolor{red}{4.22}}  \\  
        \bottomrule
    \end{tabular}
    }
    \caption{User study results for different methods across multiple evaluation metrics.}
    \label{tab:userstudy}
\end{table}

==> tabletex/table6.tex <==
\begin{table*}[ht]
    \centering
    \caption{Comparison of Computational Cost and Model Size}
    \label{tab:model_comparison}
    \begin{tabular}{l|c|c}
        \toprule
        \textbf{Method} & \textbf{FLOPs (G) \textdownarrow} & \textbf{Params (M) \textdownarrow} \\
        \midrule
        Ours & 26.465 & 1.687 \\
        BlindShadow~\cite{liu2022blind} & 2.661 & 0.784 \\
        BMNet~\cite{zhu2022bijective} & 2.750 & 0.373 \\
        DC-ShadowNet~\cite{jin2021dc} & 26.250 & 21.160 \\
        G2R-ShadowNet~\cite{liu2021shadow} & 28.470 & 22.760 \\
        DHAN~\cite{cun2020towards} & 65.720 & 21.750 \\
        Mask-ShadowGAN~\cite{hu2019mask} & 14.210 & 11.380 \\
        ST-CGAN~\cite{wang2018stacked} & 4.470 & 29.240 \\
        CIRNet~\cite{yu2024portrait} & 116.037 & 31.898 \\
        DeShadowNet~\cite{qu2017deshadownet} & 80.772 & 32.968 \\
        DMTN~\cite{liu2023decoupled} & 29.364 & 22.423 \\
        FSRNet~\cite{zhang2024frequency} & 107.633 & 167.605 \\
        HomoFormer~\cite{xiao2024homoformer} & 8.857 & 17.811 \\
        LG\_ShadowNet~\cite{liu2021shadow} & 4.419 & 3.535 \\
        Lyu \etal~\cite{lyu2022portrait} & 10.654 & 7.845 \\
        PSM~\cite{zhang2020portrait}  & 5.613 & 1.115 \\
        RASM~\cite{liu2024regional} & 6.582 & 5.156 \\
        SG\_ShadowNet~\cite{wan2022style} & 5.032 & 4.130 \\
        Shadow\_R~\cite{dong2024shadowrefiner} & 68.667 & 293.831 \\
        ShadowFormer~\cite{guo2023shadowformer} & 16.151 & 11.352 \\
        TBRNet~\cite{liu2023shadow} & 90.487 & 46.712 \\
        \bottomrule
    \end{tabular}
\end{table*}


==> tabletex/table7.tex <==
\begin{table}[h]
\centering
\small
\caption{Quantitative Summary of Shadow Diversity in ASFW }
\begin{tabular}{lccc}
\toprule
\textbf{Category} & \textbf{Sub-Type / Range} & \textbf{Sample Count} & \textbf{Proportion (\%)} \\
\midrule
\multirow{4}{*}{\textbf{Shadow Pattern Type}} 
  & Structural Shadows (e.g., nose, brow ridge)     & 256 & 23.7 \\
  & Self-occlusion Shadows (e.g., cheek folds)      & 218 & 20.2 \\
  & Occlusion Shadows (e.g., hand, hair)            & 331 & 30.6 \\
  & Accessory-Induced (e.g., hats, glasses)         & 276 & 25.5 \\
\midrule
\multirow{2}{*}{\textbf{Shadow Hardness}} 
  & Hard Shadows                  & 519 & 48.0 \\
  & Soft Shadows              & 562 & 52.0 \\
\midrule
\multirow{3}{*}{\textbf{Illumination Condition}} 
  & Frontal Lighting                                & 318 & 29.4 \\
  & Side Lighting                                   & 518 & 47.9 \\
  & Back Lighting                                   & 245 & 22.7 \\
\midrule
\multirow{4}{*}{\textbf{Shadow Area Ratio}} 
  & 0–10\% (minimal shadow)                         & 186 & 17.2 \\
  & 10–30\% (moderate shadow)                       & 303 & 28.0 \\
  & 30–50\% (large shadow)                          & 380 & 35.2 \\
  & >50\% (dominant shadow)                         & 212 & 19.6 \\
\bottomrule
\end{tabular}
\label{tab:shadow_stats}
\end{table}


==> tabletex/table8.tex <==
\begin{table*}[t]
\centering
\caption{User study results comparing the ASFW and UCB datasets. Scores are averaged over all participants. Higher is better.}
\label{tab:user_study}
\begin{tabular}{lccc}
\toprule
\textbf{Dataset} & \textbf{Shadow Naturalness} & \textbf{Color Consistency} & \textbf{Overall Quality} \\
\midrule
UCB   & 3.57 ± 0.20 & 3.56 ± 0.19 & 3.44 ± 0.10 \\
ASFW  & \textbf{4.08 ± 0.34} & \textbf{3.99 ± 0.33} & \textbf{4.04 ± 0.32} \\
\bottomrule
\end{tabular}
\end{table*}
